On monotonic determinacy and rewritability for recursive queries and views

A query Q is monotonically determined over a set of views if Q can be expressed as a monotonic function of the view image. In the case of relational algebra views and queries, monotonic determinacy coincides with rewritability as a union of conjunctive queries, and it is decidable in important special cases, such as for CQ views and queries. We investigate the situation for views and queries in the recursive query language Datalog. We give both positive and negative results about the ability to decide monotonic determinacy, and also about the co-incidence of monotonic determinacy with Datalog rewritability.

==> app-treelikeproofterm.tex <==
\section*{Proof of Proposition \ref{prop:treelikewitnessdatalog}}
Recall the statement:

\medskip

If Datalog query $Q_1$ is not  contained
in Datalog query $Q_2$, then there is instance $\inst$ and tuple $\vec d$ such
that $\inst \models  Q_1(\vec d) \wedge \neg Q_2(\vec d)$,
and a tree-like proof term  that witnesses $\inst \models  Q_1(\vec d)$, where
$\inst$ consists only of atoms in the  image of $h_{\node}$ for some node $\node$ in
the proof term.

\medskip

\begin{proof}
Let $\inst_0$ and $\vec d$ be any witness to non-containment of  $Q_1$
in $Q_2$.
Then there is a proof term $\tau$ witnesses that $\inst_0 \models  Q_1(\vec d)$.
Moving top-down on $\tau$, we form a tree-like proof term $\tau'$,  an
instance $\inst'$ that contains all the atoms in the image of mappings in $\tau'$,
 and a homomorphism from $\inst'$ to $\inst$. We will also maintain a mapping
taking atoms $A$ in $\tau$ to an atom $A'$ in $\tau'$.

At the root of the term we do not change $\tau$, we set the homomorphism
to be the identity on $\vec d$, and we let $A'$ be the same as the root atom.
In the inductive step, we consider an intensional fact
$U(\vec d)$ in $\tau_F$ witnessed by a set of facts $J$ that are a 
substitution instance of some rule body $B$. Let $U(\vec d')$ be the 
corresponding atom in $\tau'$ that we have by induction.
In $J$, we replace $\vec d$ by $\vec d'$ , and uniformly
replace any witness $w$ to an existentially quantified variable $x$ of the
rule to a fresh element $d_x$. We extend
the homomorphism to take $d_w$ to $w$, and associate any intensional fact of the body
with the corresponding fact formed by replacing $d_i$ with $d'_i$ and replacing any binding
for an existential variable $s$ with $d_x$.
\end{proof}



==> notesskrewrite.tex <==
\subsection*{Proof of Theorem \ref{thm:moncq-rewriting}}
Recall the statement:

\medskip

Suppose $Q$ is a normalized Monadic Datalog
query and $\views$ is a collection of Monadic Datalog and 
%connected 
CQ views. 
If $Q$ is monotonically determined by $\views$, then
$Q$ is rewritable over $\views$ in Datalog. The size of the rewriting is at most double-exponential in $K = O(|Q|^{|\views|})$ (``of required size'' below).

\medskip

\begin{proof}
We first argue that without any loss of generality %(see Remark~\ref{disconnected}) 
we can assume that all CQ views are connected.
If $V$ is a CQ view which is not connected, then it can be replaced by
a few connected CQs. For example, the disconnected view
$V(\vec{x},\vec{y}) = Q_1(\vec{x})\land Q_2(\vec{y})$ can be replaced by the free-variable-connected
views $V_1(\vec{x}) = Q_1(\vec{x})\land \exists \vec{y}\, Q_2(\vec{y})$ and
$V_2(\vec{y}) = (~ \exists \vec{x} \,Q_1(\vec{x})~ )\land  Q_2(\vec{y})$. Indeed, given $V$, we can restore
$V_1$ and $V_2$ as its projections on $\vec{x}$ and $\vec{y}$ respectively.
And the other way round, given $V_1$ and $V_2$, we
can restore $V$ as their product since
$V_1(\vec{x})\land V_2(\vec{y}) = Q_1(\vec{x})\land (\exists \vec{y}\, Q_2(\vec{y}))\land(\exists \vec{x} \,Q_1(\vec{x}))\land  Q_2(\vec{y})$
is equivalent in first-order logic to $Q_1(\vec{x})\land Q_2(\vec{y}) = V(\vec{x},\vec{y})$.

We need to show that there is an automaton $\automaton$ such that 
\begin{align*}
\{\views(Q_i) \mid i \in \omega\} \subseteq \decode{L(\automaton)} \subseteq 
\{\jnst \mid \views(Q_i)\text{\rm{} maps into } \jnst \text{\rm{} for some } i \in \omega\}
\end{align*}

Consider the class $\C$ of canonical databases of CQ approximations of $Q$. 
By Lemma \ref{lem:boundingtw:2} (applied with the maximal radius $r$ of the CQ views in $\views$ where  $r= O(|V|)$), the treewidth of the class $\views(\C) = \{ \views(\F) \mid \F \in \C\}$ 
of view images of $\C$ is also bounded by some $K = O(|Q|^{|\views|})$. 
By Proposition~\ref{prop:cqappr:regular},
$\C$ is $K$-regular and is captured by an NTA $\automaton^{\mathsf{base}}$ of at most exponential size in $K$.
%MICHAEL: has nothing to do with the line before it
%AND THE PROPOSITION DOES NOT SAY THIS


Without any loss of generality we assume that the sets of IDBs of programs for different views are disjoint, and that their goal predicates are
identical with the view predicates. Denote by $\Pi_{\views}$ the union of all rules in Datalog queries in $\views$, including the rules for the CQ views.
By Proposition~\ref{prop:datalog}, there is an NTA $\automaton^{\Pi_\views}$ of required size which
recognizes all codes of $\{\F \mid \F \models \Pi_{\views}, \text{tw}(\F) \le K \}$. 

We claim that the automaton $\automaton' = \automaton^{\mathsf{base}} \cap \automaton^{\Pi_\views}
$ satisfies
\begin{equation*}
\{\fpeval{\Pi_{\views}}{Q_i} \mid i \in \omega\} \subseteq \decode{L(\automaton')} \subseteq \{\F \mid \F \restr \Sigma \in \C, \F \models \Pi_{\views} \}
\end{equation*}

The proof of the first inclusion uses Lemma~\ref{lem:boundingtw:2}.
Now the automation $\automaton$ that is the projection of $\automaton'$ on the signature of view predicates 
(which exists by Proposition~\ref{prop:restriction}) captures 
$\mathbb{V} = \{ \F \restr \Sigma_\views \mid \F \restr \Sigma_{\mathbf{B}}  \in \C, \tw(\F) \le K, \F \models \Pi_\views\}$
and so satisfies two conditions of Proposition \ref{prop:backward}.
Now applying  Proposition \ref{prop:backward}, we conclude that
$Q$ is Datalog rewritable over views, and that the rewriting is of required size.
\end{proof}




